Stardust: A Scalable and Extensible Simulator for the 3D Continuum

Low Earth Orbit (LEO) satellite constellations are quickly being recognized as an upcoming extension of the Edge-Cloud Continuum into a 3D Continuum. Low-latency connectivity around the Earth and increasing computational power with every new satellite generation lead to a vision of workflows being seamlessly executed across Edge, Cloud, and space nodes. High launch costs for new satellites and the need to experiment with large constellations mandate the use of simulators for validating new orchestration algorithms. Unfortunately, existing simulators only allow for relatively small constellations to be simulated without scaling to a large number of host machines. In this paper, we present Stardust, a scalable and extensible simulator for the 3D Continuum. Stardust supports i) simulating mega constellations with 3x the size of the currently largest LEO mega constellation on a single machine, ii) experimentation with custom network routing protocols through its dynamic routing mechanism, and iii) rapid testing of orchestration algorithms or software by integrating them into the simulation as SimPlugins. We evaluate Stardust in multiple simulations to show that it is more scalable than the state-of-the-art and that it can simulate a mega constellation with up to 20.6k satellites on a single machine.

==> plots/05a-http-seq-diagram.tex <==
\begin{figure}
\resizebox{\linewidth}{!}{
  \begin{sequencediagram}
    \newthread[white]{A}{Client}
    \newinst[3.8]{B}{Stardust}{}
    \newinst[4]{C}{Real myService}{}

    \postlevel
    \begin{call}{A}{
    \shortstack{Headers: from=Vienna, \\ toService=myService}}{B}{\shortstack{reply the response \\ of real service}}
        
        \postlevel
        \begin{call}{B}{ \shortstack{wait routing latency from ground \\ station Vienna to myService}}{B}{}
        \end{call}

        \postlevel
        
        \begin{call}{B}{\shortstack{forward path, query and other \\ parameters ideally zero latency}}{C}{}
        \end{call}
        \postlevel
        
        \begin{call}{B}{\shortstack{simulate same routing \\ latency for response}}{B}{}
        \end{call}
        \postlevel
        
    \end{call}
 
  \end{sequencediagram}
  }
  \caption{HTTP proxy service to simulate realistic internet access from Node to Node or Node to Service.}
  \label{fig:Stardust:HttpSequence}
\end{figure}

==> sections/05-impl.tex <==
\section{Implementation}
\label{Stardust:sec:Impl}

The project was developed using C\# and .NET 8, the latest version of Microsoft's cross-platform development framework. Essential library functionalities for this simulator for parallel and asynchronous programming can be used and debugged quickly. The widely used Microsoft.Extensions.Hosting library simplifies the configuration of the application and supports dependency injection and more through a standardized hosting model to achieve easy modularization or adding SimPlugins. Each component is provided by dependency injection, so to replace a component just needs another implementation configured to the applications hosting provider. This simplifies the process of switching implementations and configurations of the simulation and all its components.

To demonstrate a more practical use case, an http service is implemented that acts as a routing proxy \cref{fig:Stardust:HttpSequence}. The service simply redirects client requests to a web server, mimicking basic network routing behavior. For more realistic latency modeling, the web server should be physically located close the simulation to ensure low latencies. Clients can specify in the HTTP headers the entry node into the simulated network, as well as the target node or target service they want to reach. The latency from specified node to other node or service gets applied to request and response, so the client has a realistic experience of accessing a web service through a ground node connected to the internet.

\input{plots/05a-http-seq-diagram}
